Memory-Efficient Transfer Learning with Fading Side Networks via Masked Dual Path Distillation

Memory-efficient transfer learning (METL) approaches have recently achieved promising performance in adapting pre-trained models to downstream tasks. They avoid applying gradient backpropagation in large backbones, thus significantly reducing the number of trainable parameters and high memory consumption during fine-tuning. However, since they typically employ a lightweight and learnable side network, these methods inevitably introduce additional memory and time overhead during inference, which contradicts the ultimate goal of efficient transfer learning. To address the above issue, we propose a novel approach dubbed Masked Dual Path Distillation (MDPD) to accelerate inference while retaining parameter and memory efficiency in fine-tuning with fading side networks. Specifically, MDPD develops a framework that enhances the performance by mutually distilling the frozen backbones and learnable side networks in fine-tuning, and discard the side network during inference without sacrificing accuracy. Moreover, we design a novel feature-based knowledge distillation method for the encoder structure with multiple layers. Extensive experiments on distinct backbones across vision/language-only and vision-and-language tasks demonstrate that our method not only accelerates inference by at least 25.2\% while keeping parameter and memory consumption comparable, but also remarkably promotes the accuracy compared to SOTA approaches. The source code is available at https://github.com/Zhang-VKk/MDPD.

==> CVPR26_MDPD/main_sec/0_abstract.tex <==
\begin{abstract}
Memory-efficient transfer learning (METL) approaches have recently achieved promising performance in adapting pre-trained models to downstream tasks. They avoid applying gradient backpropagation in large backbones, thus significantly reducing the number of trainable parameters and high memory consumption during fine-tuning. However, since they typically employ a lightweight and learnable side network, these methods inevitably introduce additional memory and time overhead during inference, which contradicts the ultimate goal of efficient transfer learning. To address the above issue, we propose a novel approach dubbed Masked Dual Path Distillation (MDPD) to accelerate inference while retaining parameter and memory efficiency in fine-tuning with fading side networks. Specifically, MDPD develops a framework that enhances the performance by mutually distilling the frozen backbones and learnable side networks in fine-tuning, and discard the side network during inference without sacrificing accuracy. Moreover, we design a novel feature-based knowledge distillation method for the encoder structure with multiple layers. Extensive experiments on distinct backbones across vision/language-only and vision-and-language tasks demonstrate that our method not only accelerates inference by at least 25.2\% while keeping parameter and memory consumption comparable, but also remarkably promotes the accuracy compared to SOTA approaches. {The source code is available at {\small \url{https://github.com/Zhang-VKk/MDPD}}.}
\end{abstract}

==> CVPR26_MDPD/main_sec/1_introduction.tex <==
\vspace{-0.6cm}
\section{Introduction}
\label{introduction}
Recently, large-scale pre-trained foundation models have demonstrated remarkable representation and generalization capabilities across diverse domains, including computer vision \cite{fang2023eva,he2022masked}, natural language processing \cite{radford2019language,touvron2023llama,zhuang2024towards}, and multi-modal tasks \cite{li2023blip,sun2023generative,diao2024unveiling,liang2024simple,zhang2026mingfang}. To harness strengths of these well-established models and enhance their performance towards downstream tasks, one of the most commonly used strategies is fully fine-tuning parameters of these models based on downstream datasets. However, as the number of parameters continues to vastly grow, this straightforward method becomes prohibitively computationally expensive and is prone to over-fitting, especially considering that the training data for downstream tasks is typically limited in scale. 

To deal with the above issues, parameter-efficient transfer learning (PETL) approaches \cite{houlsby2019param,hu2022lora,zhong2026hanwen} have been proposed by tuning a small number of parameters or inserting additional lightweight modules. Existing PETL methods can be roughly divided into the following three categories: 1) {Partially Tuning} \cite{guo2020parameter,sung2021training} updates a small subset of task-specific parameters while freezing the majority of the original backbone. 2) {Prompt Tuning} \cite{jia2022visual,zhou2022learning,li2021prefix,li2024multimodal} introduces a fixed number of learnable prompt vectors, which are subsequently optimized while all original parameters remain frozen. 3) {Adapter Tuning} \cite{chen2022adaptformer,chen2022vision,liao2024uni,yin20231,yin2024parameter,yin20255} incorporates additional bottleneck-shaped modules into the backbone, updating them while the backbone stays frozen. These methods significantly reduce the number of trainable parameters while achieving performance comparable to full fine-tuning. However, since the gradients are computed throughout almost the entire backbone, they still incur substantial memory consumption during training, significantly restricting their practical applicability.


Memory-efficient transfer learning (METL) \cite{zhang2020side,sung2022lst,lin2023hierarchical,mercea2024time,liu2024tuning} has recently emerged as a promising approach to achieve both parameters and memory efficiency during training. Typically, METL involves constructing a lightweight and learnable parallel side network alongside the backbone network \cite{diao2024unipt,diao2024sherl}, with static intermediate feature pairs integrated between the two at each layer. This fine-tuning paradigm reduces memory overhead by updating only the \textit{small-scale} side network while freezing the \textit{large-scale} backbone, and computing gradients exclusively for the side network during back-propagation. However, the additional forward propagation introduced by the side network result in increased inference time and memory costs, which conflicts with the ultimate goal of achieving both efficient fine-tuning and inference. %In addition, there are usually nonlinear layers (\emph{i.e.}, GELU layers) in the side branches, which are quite different from the internal structures of each layer in the backbone, and it is difficult to directly reduce the model inference time through re-parameterization technology. 

To address the aforementioned limitations, we propose a novel approach dubbed Masked Dual Path Distillation (MDPD) for memory-efficient transfer learning based on the side network framework. Without compromising inference speed, MDPD distills intermediate features from the backbone and the final output of the side network separately, while efficiently guiding and updating the backbone through the lightweight side network, thereby reducing training memory overhead. Specifically, during training, feature- and logits-based knowledge distillation methods are applied to the intermediate features of the backbone and the final logits output of the side network. In a dual-path framework, alternating optimization of the backbone and the side network minimizes their discrepancy in feature distributions. During inference, only the optimized backbone is utilized, eliminating additional inference time while maintaining the performance, thus achieving efficiency in both training memory and inference speed. Furthermore, previous feature distillation strategies often require the student model to directly mimic the intermediate features of the teacher model. Nevertheless, the feature distributions of these two models typically differ, particularly in the attentive areas of the input, making direct imitation challenging. Additionally, existing methods usually only distill a subset of the layers or even just the final layer of the teacher or student network. For backbones with multiple encoding layers such as ViT and BERT, where deep and shallow layers focus on different tokens, it is equally important to perform distillation in the deep and shallow layers. Therefore, We also propose a novel feature-based distillation strategy by applying direct imitation in the shallow layer of the backbone, while employing mask generation in the deep layers, ensuring more effective and balanced distillation.

%In order to fully evaluate the generalization of our method, we tested the effectiveness of our method on five challenging visual-language tasks and a pure-vision benchmark. The experimental results show that our method outperforms other state-of-the-art METL methods with comparable training consumption and lower inference cost, \emph{i.e.}, it achieves the best balance between performance and parameter/memory/time efficiency.

The main contributions of this work lie in three-fold:

(1) We propose Masked Dual Path Distillation (MDPD), a novel approach designed to accelerate current METL frameworks, which introduces the side networks to guide backbone optimization with mutual distillation during training, while discarding them during inference to enhance efficiency without compromising accuracy.

(2) We develop a Hierarchical Feature-based Distillation method by employing tailored  distillation strategies for distinct layers to mitigate the discrepancies between the backbone and side networks. 

(3) We extensively evaluate our method across multiple visual-language and vision/language-only tasks based on distinct backbones, demonstrating that our approach remarkably reduces the inference time by at least 22.5\%, while maintaining accuracy as well as memory and parameter efficiency.


==> CVPR26_MDPD/main_sec/2_related_work.tex <==
\section{Related Work}
\label{related_work}

\subsection{Parameter-Efficient Transfer Learning}
Pre-trained foundation models have achieved remarkable success across various domains~\cite{devllin2019bert, liu2019roberta, alexey2021vit, radford2021learning, girdhar2023image,wu2026zimeng}. However, their application to downstream tasks encounters challenges in computational efficiency and adaptability, sparking significant interest in parameter-efficient transfer learning (PETL) techniques. Existing PETL methods roughly fall into the following categories. 1) \emph{Selective tuning} methods update only a subset of parameters, such as bias \cite{cai2020tinytl, zaken2022bitfit}, weights \cite{zhao2020masking, touvron2022three} and normalization layers \cite{kim2021howto}, while freezing the rest. 2) \emph{Additive methods} introduce additional parameters and focus on training them instead of backbones, including Adapter-based ones \cite{houlsby2019param, zhu2021counter, he2022sparse, he2022towards, he2023sensitivity,chen2026zhenghao} and Prompt tuning based ones \cite{hambardzumyan2021warp, lester2021power, li2021prefix, vu2021spot, qin2022exploring}. (3) \emph{Re-parameterized} methods \cite{hu2022lora, he2023param, song2024increasing, wu2024mixture, wu2025unified,zhong2024hanwen} employ extra trainable parameters with low-rank structures to reduce computational cost.

\subsection{Memory-Efficient Transfer Learning}
Different from PETL that aims to reduce trainable parameters, memory-efficient transfer learning (METL) focuses on decreasing memory consumption during training. Typically, \cite{zhang2020side, sung2022lst, jiang2024res, diao2024unipt, diao2024sherl, zhang2026moismoe} accomplish memory-efficient tuning by introducing learnable side network parallel to the backbone \cite{zhang2020side, sung2022lst, jiang2024res, diao2024unipt, diao2024sherl}, which confine back-propagation to side network. It avoids storing gradients of large-scale backbones, thereby reducing memory overhead. 
% Among these methods, UniPT \cite{diao2024unipt} incorporates a parallel interaction module to independently process intermediate outputs of each layer, alongside a confidence aggregation module that adaptively determines optimal strategies for integrating features across layers. Similarly, SHERL \cite{diao2024sherl} employs an anti-redundancy mechanism to consolidate intermediate outputs, subsequently transforming these flexible features into more robust and adaptive representations. 
Alternatively, \cite{liao2023make}, leverages reversible models \cite{gomez2017reversible, zhang2023lora-fa} by enabling activations to be recomputed during back-propagation rather than being stored during the forward pass. Some works \cite{malladi2023tune, phang2023hypertuning} attempt to avoid back-propagation.
% Similarly, LoRA-FA \cite{zhang2023lora-fa} focuses on updating only the projection-up weight within each LoRA layer, and removing the need to store input activations. 
% such as HyperTuning \cite{phang2023hypertuning}, which employs a hypermodel to generate PEFT parameters based on few-shot examples, and MeZO \cite{malladi2023tune}, which uses a zeroth-order gradient estimator to approximate the gradient during the forward pass, both enabling efficient fine-tuning without back-propagation. 
Besides, \cite{gomez2017reversible,2016Training}
reconstruct discarded activations from backward layers or perform gradient checkpoint operation without storing all intermediate activations, and \cite{gomez2017reversible}. Despite memory efficient, these methods significantly limit the model capacity and lag far behind the performance of full fine-tuning.

\subsection{Knowledge Distillation}
Knowledge distillation (KD) \cite{hinton2015distilling,pan2024disentangled} trains a smaller student model to mimic the larger teacher model, which can be categorized into logits-based, feature-based and relation-based methods. 1) \emph{Logits-based} methods \cite{meng2019conditional, wu2022tinyvit} focus on mimicing the final output of the teacher model.
% with representative approaches including conditional T/S learning \cite{meng2019conditional}  and TinyViT \cite{wu2022tinyvit}.
2) \emph{Feature-based} methods \cite{romero2015fitnets, chen2021cross, bai2023masked} leverage the intermediate representations of  teacher networks to guide the learning process of student networks.
% with notable methods including FitNet \cite{romero2015fitnets}, SemCKD \cite{chen2021cross} and DMAE \cite{bai2023masked}.
3) \emph{Relation-based} methods \cite{yim2017gift, chen2021learning, chen2024joint} explore relationships between different layers of teacher models as knowledge, which is utilized to facilitate learning of student models.
% with representative techniques such as FSP \cite{yim2017gift} and LP \cite{chen2021learning}.

==> CVPR26_MDPD/main_sec/3_methodology.tex <==
\begin{figure*}[!t]
% \vspace{-0.5cm}
\centering
\includegraphics[width=0.98\textwidth]{figures/framework.pdf} 
%\caption{Illustration on the proposed framework. Part (I) shows Masked Dual Path Distillation for side network based universal METL. Specifically, during the training stage, most of the parameters of the backbone are frozen, while the parameters of the Layer Normalization of each layer and side network are updated. The two networks take turns to act as the teacher and student models respectively, performing knowledge distillation on the intermediate layer features and output logits, using the side branch to efficiently guide the training of the backbone, while only enabling the gradients returned by the side branch to expeditiously update the backbone. During the inference stage, the side branch is discarded and only the backbone is used for reasoning to improve the inference speed. Part (II) shows Hierarchical Feature-based Distillation. For encoder structures with multiple layers, when performing feature-based distillation on the intermediate features of the teacher and student model, we directly imitate at the shallow layer and use a generative approach at the deep layer. It can also be directly combined with other logits-based distillation methods.}
\caption{Illustration on our method. Part (I) shows the pipeline of Masked Dual Path Distillation. During training, the backbone and side networks mutually act as teacher and student for effective distillation, where side networks are abandoned after training for inference efficiency. Part (II) displays Hierarchical Feature-based Distillation that adopt distinct strategies across different layers. It particularly selects a set of masked features, making them learnable with guidance of backbones in deep layers. %using the side branch to efficiently guide the training of the backbone, while only enabling the gradients returned by the side branch to expeditiously update the backbone. During the inference stage, the side branch is discarded and only the backbone is used for reasoning to improve the inference speed. Part (II) shows Hierarchical Feature-based Distillation. For encoder structures with multiple layers, when performing feature-based distillation on the intermediate features of the teacher and student model, we directly imitate at the shallow layer and use a generative approach at the deep layer. It can also be directly combined with other logits-based distillation methods.
}
\label{fig-framework}
% \vspace{-0.5cm}
\vspace{-0.3cm}
\end{figure*}

\section{Methodology}
\subsection{Framework Overview}
\label{overview}
Generally, previous METL methods significantly reduce training memory overhead by constructing a lightweight, trainable side network to avoid gradients directly passing through a large backbone. Similar to the structure of backbone, side network is usually composed of several intermediate layers and initialized by pre-trained weights. However, the corresponding layers of two networks cannot be fully forward propagated parallelly, as the input of the side network branch is guided by the output of the intermediate layer or final layer of backbone. Therefore, during the forward pass of the model, the side branch inevitably introduces additional computational overhead in both training and inference, ultimately reducing the overall efficiency. To address this issue, we propose a novel method dubbed Masked Dual Path Distillation (MDPD) as shown in Fig.~\ref{fig-framework}.
% which can achieve a better balance between model capacity, training memory, and inference time. Inspired by knowledge distillation, we consider distilling all the knowledge learned by side network into nearly frozen pre-trained backbone during, and guiding parameters of Layer Normalization of backbone to update, so that it learn side knowledge during training phase without storing more intermediate activations. 

Specifically, given a single modality input $\mathcal{X}$, a pre-trained backbone $\Phi_{1:L}$ containing $L$ layers is used to extract $L$ token sequences $\bm{b}^1,\cdots,\bm{b}^L\in\mathbb{R}^{N\times D_B}$, each consisting of $N$ tokens with a hidden dimensionality of $D_B$. After obtaining final output $\bm{b}^L$ of backbone, it is fused with each intermediate sequences $\bm{b}^l,l\in 1,2,\cdots,L-1$ and regarded as corresponding layer input of side network, which also contains $L$ layers $\Theta_{1:L}$, to extract side token sequences $\bm{s}^1,\cdots,\bm{s}^L\in \mathbb{R}^{N\times D_S}$, usually consisting of $N$ $D_S$-dimensional ($D_S{<D_B}$) tokens. Subsequently, in order to utilize powerful model representation ability of pre-trained network, backbone and side network is regarded as teacher $\mathcal{T}_{fea}$ and student $\mathcal{S}_{fea}$ model respectively, and intermediate features of corresponding layers $\bm{b}^l$ and $\bm{s}^l$ are distilled to enhance feature extraction ability of side branch. In particular, when performing feature-based distillation on an encoder structure which containing multiple layers, we find that there are significant differences in attention pattern of teacher-student network at different layers. For shallow layers of the network, attention map of students and teachers is diagonal, showing a \textit{self-attention} pattern; while for deep layers, attention patterns gradually diverge, and begin to focus on different sparse key tokens respectively. This difference makes it difficult for students to directly imitate distribution of teacher's final features. Therefore, in response to above findings, we fine-grain knowledge distillation strategies for different layers. Specifically, for shallow layers with smaller differences, students are forced to directly mimic features of corresponding layers of teacher and learn how to focus on the tokens themselves; for deep layers with larger differences and stronger semantic information, students are forced to generate features of teacher rather than directly imitate them. In addition, since only final layer features of side network are used as the final output of the model during the training stage, and backbone is not considered (\emph{i.e.}, the backbone is not followed by a task-specific head), we manually design a new output layer, while regard backbone and side network as a student $\mathcal{S}_{log}$ and teacher $\mathcal{T}_{log}$ model respectively for logits-based distillation, which is performed on final outputs of two networks $\mathbf{b}_L$ and $\mathbf{s}_L$ and transfer knowledge of side network to backbone to optimize latter's model output performance. {At training stage, most of parameters in backbone remain frozen to prevent a large amount of gradients from flowing through, and only scaling and shifting coefficients of Layer Normalization in each block and parameters of final output layer are updated, while all parameters in side network are learnable as well.} In inference stage, backbone equipped with a task-specific head is directly used to perform inference operations, while side branch is discarded directly, thereby achieving parameter- and memory-efficient training and time-efficient inference, and gain better performance.

\subsection{Dual Path Knowledge Distillation}
\label{dual_path}

In order to enable backbone to have the ability of independent inferring, we propose a Dual Path Knowledge Distillation (DPKD) strategy, which aims to distill the downstream task-specific knowledge learned by the side network into backbone, so as to be efficiently guided and updated. In order to make full use of prior knowledge of pre-trained backbone and enable side network to obtain a stronger model representation capacity, based on knowledge distillation, we first adopt feature-based distillation to calculate distillation loss for corresponding intermediate layer features of backbone and side network. Specifically, backbone $B$ and side network $S$ are regarded as teacher $\mathcal{T}_{fea}$ and student $\mathcal{S}_{fea}$, respectively. After obtaining $l$-th layer features of backbone $\bm{b}^l\in\mathbb{R}^{N\times D_B}$ and side branch $\bm{s}^l\in\mathbb{R}^{N\times D_S} (D_S<D_B)$, hidden dimensions need to be aligned firstly in order to perform distillation operation. However, if a $1 \times 1$ convolutional layer is used to implement alignment operation, approximately $(1+D_B)\times D_S$ parameters will be introduced, which violates the goal of parameter-efficiency. Therefore, we consider using two low-rank matrices $\bm{M}_{down}\in \mathbb{R}^{D_S\times d}$ and $\bm{M}_{up}\in \mathbb{R}^{d\times D_B}$ in the form of a bottleneck, first reducing $D_S$ to a lower dimension $d (d\ll \min(D_B,D_S))$, and then increasing it to $D_B$:
\begin{equation}
    \phi(\bm{s}^l)=\bm{s}^l\bm{M}_{down}\bm{M}_{up} \Rightarrow \bm{b}^l,
\end{equation}
where $l\in 1,2,\cdots,12$ represents the layer index, $\phi(\cdot)$ is the bottleneck module used to reshape the dimension of $\bm{s}^l$ to the same as $\bm{b}^l$. This will only introduce about $(1+D_S+D_B)\times d+D_B$ parameters, but still be able to obtain comparable or even better experimental results than a single convolutional layer, while ensuring parameter- and memory-efficiency. Then, we calculate the distillation loss $\mathcal{L}_{\text{fea}}$ for the intermediate features of each layer:
\begin{equation}\label{feature_loss}
    \mathcal{L}_{\text{fea}}^l=\sum_{i=1}^{N}\sum_{j=1}^{D_B}(\bm{b}^l_{i,j}-\phi(\bm{s}^l)_{i,j})^2,
\end{equation}
where $N$,$D_B$ represent the number of tokens and hidden dimensions of teacher's feature, respectively. After feature-based distillation, side branch obtains stronger representation capability under the guidance of pre-trained backbone, thus can mine richer and more important features.

In addition, as the output of side network is final output of the model without the contribution of backbone, so as to ensure that only the backbone is used for inferring, a strong task-related mapping layer is required to obtain final logits. We first use global average pooling (GAP) on final feature maps of backbone and side branch $\bm{b}^L$ and $\bm{s}^L$, then adopt linear mapping layers $\bm{W}_B$ and $\bm{W}_S$ to get output logits of two networks $\mathcal{Y}^B\in\mathbb{R}^{D_B'}$ and $\mathcal{Y}^S\in\mathbb{R}^{D_S'}$, respectively. Successively, side network and backbone are regarded as teacher $\mathcal{T}_{log}$ and student $\mathcal{S}_{log}$ respectively, and we adopt logits-based distillation strategy to calculate loss $\mathcal{L}_{\text{log}}$ for $\mathcal{Y}^B$ and $\mathcal{Y}^S$: 
\begin{equation}\label{logits_loss}
    % \vspace{-0.3cm}
    \mathcal{L}_{\text{log}}=\sum_{i=1}^{D_S'}(\mathcal{Y}^S_{i}-\phi(\mathcal{Y}^B)_{i})^2,
    % \vspace{-0.2cm}
\end{equation}
After logits-based distillation, the output layer of the backbone can independently obtain stronger mapping ability in the inference stage under the guidance of the side branch, thereby showing better model performance.

{In the above process, the backbone $B$ and the side network $S$ take turns as teacher or student models. Through the Dual Path Knowledge Distillation method, they teach each other the knowledge of their own strong parts and learn from each other the knowledge of their own weak parts. The two guide each other and achieve alternating optimization.} Therefore, in the inference stage, only the backbone is used for inferring and the side network is discarded. While avoiding introducing additional inference time, the model can still maintain a better performance, thereby achieving a balance between performance, parameters, memory, and time. 

\subsection{Hierarchical Feature-based Distillation}
\label{feature_distill}

As teacher and student networks typically exhibit similar attention patterns in shallow layers, we guide student to align with teacher's distribution. Specifically, we adopt the following loss in shallow layers:
% as in Eq. \eqref{feature_loss}, a bottleneck module is first used to align hidden dimensions of the student's and teacher's features, and 
%$\mathcal{L}_{\text{sha}}$ is expressed as:
\begin{equation}
    \mathcal{L}_{\text{sha}}^l=\sum_{i=1}^{N}\sum_{j=1}^{D_B}(\bm{b}^l_{i,j}-\phi(\bm{s}^l)_{i,j})^2.
\end{equation}

In deep layers, features of teacher and student networks often have significantly varying attention patterns, making direct distillation infeasible. Therefore, we try to force the student to fit the distribution of the teacher's features through generation. Generally, deep features contain rich semantic information. At the same time, the tokens of such features also contain information about adjacent tokens. Therefore, we use the student's masked features to generate the teacher's features, which only use partial tokens to represent the complete original attention map. This can not only retain some of the original student feature information, but also obtain a better feature representation through generation. Similarly, we first use a bottleneck module to align the hidden dimensions of the student's and teacher's features. {Then, we set a set of shared random mask values $\bm{m}\in\mathbb{R}^{N\times 1}$ to specify the coordinates of the student's original feature tokens replaced by the learnable mask tokens:}
\begin{equation}
\label{eq:mask}
    \bm{m}_i=
    \begin{cases}
        1,\enspace {\rm{if}}~~~r_i<\lambda, \\
        0,\enspace \rm{otherwise},
    \end{cases}
\end{equation}
where $r_i\in [0,1]$ is a random number deciding whether the $i$-th token is masked. {$\lambda$ is the ratio controlling the proportion of masking, which is unitarily applied to all deep layers of side network.} Based on $\bm{m}_i$, we update features of student network as below:
\begin{equation}
    \bar{\bm{s}}_i=
    \begin{cases}
        \bm{f}_{mask},\enspace {\rm{if}}~~~\bm{m}_i, \\
        \bm{f}_{ori},\enspace \rm{otherwise},
    \end{cases}
\end{equation}
where $\bm{f}_{ori}$ is the the original features and  $\bm{f}_{mask}$ is the learnable masked feature. Then, we utilize $\bar{\bm{s}}$ to generate the teacher's features with a generation block $\mathcal{G}(\cdot)$, which is a projector with two 3$\times$3 convolutional layers and one ReLU activation layer. Finally, the loss of feature-based distillation in deep layers $\mathcal{L}_{\text{deep}}$ is expressed as:
\begin{equation}
\label{eq:generation_block}
\mathcal{L}_{\text{deep}}^l=\sum_{i=1}^{N}\sum_{j=1}^{D_B}\bm{m}_i\cdot (\bm{b}^l_{i,j}-\mathcal{G}(\bar{\bm{s}^l})_{i,j})^2.
\end{equation}

==> CVPR26_MDPD/main_sec/4_experimental.tex <==
\section{Experimental Results and Analysis}
\label{experiment}

\subsection{Experimental Setup}

\textbf{Dataset.}
We primarily evaluate performance of our method on various \emph{vision-language (VL) tasks}, including:
(1) Image-Text Retrieval ($\textbf{ITR}$) on Flickr30K \cite{young2014image} and MSCOCO \cite{lin2014microsoft}; (2) Video-Text Retrieval ($\textbf{VTR}$) on MSVD \cite{chen2011collecting} and MSR-VTT \cite{xu2016msr}; (3) Question Answering ($\textbf{VQA\&GQA}$) on VQAv2 \cite{goyal2017making} and GQA \cite{hudson2019gqa}; and (4) Visual Grounding ($\textbf{VG}$) on RefCOCO, RefCOCO+ \cite{yu2016modeling} and RefCOCOg \cite{mao2016generation}. Additionally, we evaluate our approach on \emph{vision-only and language-only tasks} on \textbf{VTAB-1K} \cite{zhai2019large} and \textbf{GLUE} benchmark \cite{wang2018glue}, respectively. 
% For the former, we report results on \textbf{VTAB-1K} \cite{zhai2019large}, which comprises 19 datasets across various subtasks designed for efficient transfer learning. For the later, we evaluate on the \textbf{GLUE} benchmark \cite{wang2018glue} across distinct tasks, including: (1) linguistic acceptability on CoLA \cite{warstadt2019neural}; (2) sentiment analysis on SST2 \cite{socher2013recursive}; (3) similarity and paraphrase on MRPC~\cite{dolan2005automatically}, QQP and STS-B \cite{cer2017semeval}; and (4) natural language inference on MNLI \cite{williams2017broad}, QNLI \cite{rajpurkar2016squad} and RTE \cite{bentivogli2009fifth}.

\noindent\textbf{Evaluation Metrics.}
We report Recall@1 and Rsum on ITR and VTR tasks, overall Accuracy on QA tasks, and mean Average Precision on VG tasks. For GLUE benchmark, we present Accuracy Metric, F1 Score, Matthew's Correlation, Pearson-Spearman Correlation as the evaluation metrics for various datasets respectively. Besides, we state Top-1 Accuracy on 19 datasets in VTAB-1K. More details are in \textit{Supplementary Material}. 
Besides, we report GPU memory usage (G) during training, number of trainable parameters (M), and inference latency (ms per run), FPS (frames per second) or QPS (queries per second) as efficiency metrics.
% Following existing works \cite{diao2024unipt}, for ITR and VTR, we report Recall@1 (R@1) for sentence retrieval (I-T, V-T), image retrieval (T-I), and video retrieval (T-V), along with the Rsum of R@1/5/10 across both directions for comprehensive evaluation. For VQA and GQA, we present the overall accuracy on the Test-Dev (Test$_\text{Dev}$) and Test-Std (Test$_\text{Std}$) dataset splits. In the case of VG, mean Average Precision (mAP) is evaluated on validation images (Val), test images containing multiple people (TestA) and on test images with multiple instances of all other objects (TestB). For VTAB-1K \cite{zhai2019large}, we report the averaged accuracy across distinct datasets. In regards of GLUE \cite{wang2018glue}, we report accuracy on SST-2/MNLI/QNLI/RTE, Matthew's Correlation on CoLA, Pearson-Spearman Correlation on STS-B, and the average of F1 score and accuracy on MRPC/QQP, respectively. Besides accuracy, we also report metrics on efficiency, including GPU memory usage (G) during training, number of trainable parameters (M), and inference latency (ms per run).


\noindent\textbf{Implementation Details.}
To ensure fair comparisons, we follow \cite{diao2024unipt,diao2024sherl} by aligning most settings with the original pre-trained models, including the optimizer, warm-up scheduler, batch size, training epochs, \emph{etc}. More details are provided in \textit{Supplementary Material}.
% To ensure fair comparisons, we follow existing works by aligning most settings with the original pre-trained models, including the optimizer, image size and training epochs. For the ITR task using VSE$\infty$, we set the batch size to 112, while maintaining consistency with pre-trained models for all other tasks. For vision-language tasks, we adjust these hyperparameters by following \cite{diao2024sherl}, scaling learning rate by a factor of 10, and setting the reduction factor and mask rate $\lambda$ to 2 and 0.5, respectively. For language-only tasks, similar to \cite{sung2022lst}, we set learning rate and reduction factor to $3 \times 10^{-3}$ and 8, respectively. All experiments are conducted on an NVIDIA GeForce RTX 3090Ti GPU. More details are provided in the \textit{Supplementary Material}.

%each method undergoes training with 20 epochs on small datasets and 10 epochs for the rest large ones

\begin{table*}[t]
    \centering
    \caption{Comparison results with PETL \textbf{(Middle)} and METL \textbf{(Bottom)} approaches across distinct network architectures. Best results are in \textbf{bold}, and second best results are \underline{underlined}.}
    \vspace{-0.1cm}
    \small
    \setlength{\tabcolsep}{1.9pt}
    \scalebox{0.95}{
    \begin{tabular}{lcccccc|cccccc|cccccc}
    \toprule
    
    \multirow{2}{*}{Method} & Params. & Mem. & QPS & \multicolumn{3}{c|}{BERT+BUTD} & Params. & Mem. & QPS & \multicolumn{3}{c|}{ResNeXt+BiGRU} & Params. & Mem. & QPS & \multicolumn{3}{c}{ViT+Text Transf.} \\
        \cmidrule[0.4pt]{5-7} \cmidrule[0.4pt]{11-13} \cmidrule[0.4pt]{17-19}
        & (M) $\!\downarrow$ & (G) $\!\downarrow$ & $\!\uparrow$ & I-T $\!\uparrow$ & T-I $\!\uparrow$ & Rsum $\!\uparrow\ $ & (M) $\!\downarrow$ & (G) $\!\downarrow$ & $\!\uparrow$ & I-T $\!\uparrow$ & T-I $\!\uparrow$ & Rsum $\!\uparrow\ $ & (M) $\!\downarrow$ & (G) $\!\downarrow$ & $\!\uparrow$ & T-V $\!\uparrow$ & V-T $\!\uparrow$ & Rsum $\!\uparrow$ \\
    
    \midrule

    \textcolor{gray}{Fully-FT} & \textcolor{gray}{109.5} & \textcolor{gray}{9.9} & \textcolor{gray}{24.14} & \textcolor{gray}{79.7}  & \textcolor{gray}{62.1} & \textcolor{gray}{513.5}  & \textcolor{gray}{90.9} & \textcolor{gray}{174.4} & \textcolor{gray}{30.80} & \textcolor{gray}{85.6} & \textcolor{gray}{70.2} & \textcolor{gray}{539.0}  & \textcolor{gray}{151.3} & \textcolor{gray}{48.8} & \textcolor{gray}{44.07} & \textcolor{gray}{42.8} & \textcolor{gray}{42.1} & \textcolor{gray}{389.2} \\
        \textcolor{gray}{Partially} & \textcolor{gray}{0.8} & \textcolor{gray}{1.0} & \textcolor{gray}{24.19} & \textcolor{gray}{74.8} & \textcolor{gray}{57.3} & \textcolor{gray}{485.5}  & \textcolor{gray}{2.1} & \textcolor{gray}{14.9} & \textcolor{gray}{31.26} & \textcolor{gray}{75.2} & \textcolor{gray}{58.2} & \textcolor{gray}{505.8} & \textcolor{gray}{0.7} & \textcolor{gray}{7.6} & \textcolor{gray}{44.48} & \textcolor{gray}{36.4} & \textcolor{gray}{37.0} & \textcolor{gray}{353.9} \\
        \midrule[0.6pt]
        Adapter \cite{houlsby2019param} & 2.6 & 8.8 & 22.44 & 79.1  & \underline{60.5} & \underline{511.3}  & 3.5 & 176.8 & 28.65 & 66.8 & 62.9 & 493.3  & 5.2 & 41.2 & 39.17 & 38.3 & 39.6 & 364.3 \\
        LoRA \cite{hu2022lora} & \underline{1.1} & 8.8 & 23.37 & 78.8 & 59.6 & 508.2  & -- & -- & -- & -- & -- & --  & 1.3 & 40.8 & 41.55 & 38.8 & 39.9 & 366.8 \\
        BitFit \cite{zaken2022bitfit}  & 0.9 & 8.6 & \underline{23.70} & 77.3 & 57.8 & 503.9  & \underline{2.2} & 168.0 & \underline{30.53} & 83.4 & 67.4 & 530.6 & \textbf{0.1} & 42.0 & \underline{43.12} & 38.1 & 40.6 & \underline{370.8} \\
        Prompt \cite{li2021prefix} & 10.7 & 9.4 & 17.64 & 78.7 & 59.0 & 508.5  & -- & -- & -- & -- & -- & --  & \underline{0.2} & 42.8 & 33.74 & 36.8 & 37.5 & 358.8 \\
        SSF \cite{lian2022scaling} & \textbf{0.2} & 8.4 & 22.23 & 80.0 & 60.4 & 512.8  & \textbf{0.1} & 163.2 & 27.63 & 83.7 & 66.8 & 528.5  & 0.5 & 39.2 & 37.91 & \textbf{40.2} & \textbf{41.8} & \textbf{376.6} \\
        FacT \cite{jie2023fact} & 0.6 & 8.7 & -- & 79.2 & 59.3 & 508.8  & -- & -- & -- & -- & -- & --  & 0.8 & 40.8 & -- & 38.7 & 39.8 & 367.2 \\
        AdaLoRA \cite{zhang2023adaptive} & 1.0 & 8.8 & 23.03 & 79.8 & 60.1 & 510.3  & -- & -- & -- & -- & -- & --  & 1.2 & 42.0 & 40.06 & \underline{39.2} & 39.6 & 368.5 \\
        \midrule[0.6pt]
        LST \cite{sung2022lst} & 7.5 & 4.6 & 10.73 & 77.9 & 57.3 & 501.9 & 2.3 & \textbf{15.0} & 13.86 & 82.3 & 66.1 & 526.7  & 11.2 & 32.0 & 19.85 & 37.0 & 37.8 & 356.7 \\
        UniPT \cite{liao2024uni} & 5.9 & \textbf{3.1} & 12.75 & \underline{80.2} & 59.8 & 510.5 & 6.4 & \textbf{15.0} & 17.83 & \underline{84.0} & \underline{67.7} & \underline{532.1}  & 9.6 & \textbf{13.6} & 27.03 & 38.9 & 39.3 & 361.3 \\
        
        \textbf{Ours} & 5.9  & \underline{3.4} & \textbf{24.05} & \textbf{81.9} & \textbf{61.1} & \textbf{516.2} & 6.5 & \underline{15.7} & \textbf{30.62} & \textbf{85.3} & \textbf{69.8} & \textbf{539.1} & 9.7 & \underline{14.0} & \textbf{43.52} & \textbf{40.2} & \underline{40.7} & 365.8 \\
    
    \bottomrule
    \end{tabular}
    }
    \label{tab1}
    \vspace{-0.2cm}
\end{table*}

% \begin{table*}[!t]
% % \vspace{-0.2cm}
% %Comparative Analysis of Parameter, Memory Usage, Inference Time Consumption, and Task Performance across CNN, Single Transformer, and Dual Transformer Architectures. We evaluates various methods using metrics such as parameters, memory utilization, inference time and retrieval outcomes. Results highlight the balance between computational efficiency and task performance, with the best-performing results emphasized in \textbf{BOLD} and the second best is \underline{UNDERLINED}.
%     \begin{center}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l c c c ccc | c c c ccc | c c c ccc}
%         \toprule[1.2pt]
%         {\multirow{2}{*}{Method}} & Params. & Memory & Time & \multicolumn{3}{c|}{BERT} & Params. & Memory & Time & \multicolumn{3}{c|}{ResNeXt-101} & Params. & Memory & Time & \multicolumn{3}{c}{ViT + Text Transf.} \\
%         \cmidrule[0.4pt]{5-7} \cmidrule[0.4pt]{11-13} \cmidrule[0.4pt]{17-19}
%         {} & (M) \downarrow & (G) \downarrow & (ms) \downarrow & I-T \uparrow & T-I \uparrow & Rsum \uparrow & (M) \downarrow & (G) \downarrow & (ms) \downarrow & I-T \uparrow & T-I \uparrow & Rsum \uparrow & (M) \downarrow & (G) \downarrow & (ms) \downarrow & T-V \uparrow & V-T \uparrow & Rsum \uparrow \\
%         \midrule[0.6pt]
%         \textcolor{gray}{Fully-FT} & \textcolor{gray}{109.5} & \textcolor{gray}{9.9} & \textcolor{gray}{41.42} & \textcolor{gray}{79.7}  & \textcolor{gray}{62.1} & \textcolor{gray}{513.5}  & \textcolor{gray}{90.9} & \textcolor{gray}{174.4} & \textcolor{gray}{32.47} & \textcolor{gray}{85.6} & \textcolor{gray}{70.2} & \textcolor{gray}{539.0}  & \textcolor{gray}{151.3} & \textcolor{gray}{48.8} & \textcolor{gray}{22.69} & \textcolor{gray}{42.8} & \textcolor{gray}{42.1} & \textcolor{gray}{389.2} \\
%         \textcolor{gray}{Partially} & \textcolor{gray}{0.8} & \textcolor{gray}{1.0} & \textcolor{gray}{41.34} & \textcolor{gray}{74.8} & \textcolor{gray}{57.3} & \textcolor{gray}{485.5}  & \textcolor{gray}{2.1} & \textcolor{gray}{14.9} & \textcolor{gray}{31.99} & \textcolor{gray}{75.2} & \textcolor{gray}{58.2} & \textcolor{gray}{505.8} & \textcolor{gray}{0.7} & \textcolor{gray}{7.6} & \textcolor{gray}{22.48} & \textcolor{gray}{36.4} & \textcolor{gray}{37.0} & \textcolor{gray}{353.9} \\
%         \midrule[0.6pt]
%         Adapter \cite{houlsby2019param} & 2.6 & 8.8 & 44.57 & 79.1  & \underline{60.5} & \underline{511.3}  & 3.5 & 176.8 & 34.91 & 66.8 & 62.9 & 493.3  & 5.2 & 41.2 & 25.53 & 38.3 & 39.6 & 364.3 \\
%         LoRA \cite{hu2022lora} & \underline{1.1} & 8.8 & 42.79 & 78.8 & 59.6 & 508.2  & -- & -- & -- & -- & -- & --  & 1.3 & 40.8 & 24.07 & 38.8 & 39.9 & 366.8 \\
%         BitFit \cite{zaken2022bitfit}  & 0.9 & 8.6 & \underline{42.19} & 77.3 & 57.8 & 503.9  & \underline{2.2} & 168.0 & \underline{32.76} & 83.4 & 67.4 & 530.6 & \textbf{0.1} & 42.0 & \underline{23.19} & 38.1 & 40.6 & \underline{370.8} \\
%         Prompt \cite{li2021prefix} & 10.7 & 9.4 & 56.70 & 78.7 & 59.0 & 508.5  & -- & -- & -- & -- & -- & --  & \underline{0.2} & 42.8 & 29.64 & 36.8 & 37.5 & 358.8 \\
%         SSF \cite{lian2022scaling} & \textbf{0.2} & 8.4 & 44.98 & 80.0 & 60.4 & 512.8  & \textbf{0.1} & 163.2 & 36.19 & 83.7 & 66.8 & 528.5  & 0.5 & 39.2 & 26.38 & \textbf{40.2} & \textbf{41.8} & \textbf{376.6} \\
%         FacT \cite{jie2023fact} & 0.6 & 8.7 & -- & 79.2 & 59.3 & 508.8  & -- & -- & -- & -- & -- & --  & 0.8 & 40.8 & -- & 38.7 & 39.8 & 367.2 \\
%         AdaLoRA \cite{zhang2023adaptive} & 1.0 & 8.8 & 43.42 & 79.8 & 60.1 & 510.3  & -- & -- & -- & -- & -- & --  & 1.2 & 42.0 & 24.96 & \underline{39.2} & 39.6 & 368.5 \\
%         \midrule[0.6pt]
%         LST \cite{sung2022lst} & 7.5 & 4.6 & 93.17 & 77.9 & 57.3 & 501.9 & 2.3 & \textbf{15.0} & 72.15 & 82.3 & 66.1 & 526.7  & 11.2 & 32.0 & 50.37 & 37.0 & 37.8 & 356.7 \\
%         UniPT \cite{diao2024unipt} & 5.9 & \textbf{3.1} & 78.41 & \underline{80.2} & 59.8 & 510.5 & 6.4 & \textbf{15.0} & 56.09 & \underline{84.0} & \underline{67.7} & \underline{532.1}  & 9.6 & \textbf{13.6} & 36.99 & 38.9 & 39.3 & 361.3 \\
%         \textbf{Ours} & 5.9  & \underline{3.4} & \textbf{41.58} & \textbf{81.9} & \textbf{61.1} & \textbf{516.2} & 6.5 & \underline{15.7} & \textbf{32.66} & \textbf{85.3} & \textbf{69.8} & \textbf{539.1} & 9.7 & \underline{14.0} & \textbf{22.98} & \textbf{40.2} & \underline{40.7} & 365.8 \\
%         \bottomrule[1.2pt]
%     \end{tabular}}
%     \end{center}
%     \caption{Comparison results with memory inefficient PETL approaches across Single Transformer (BERT), CNN (ResNeXt-101) and Dual Transformer (ViT + Text Transformer) network architectures, in terms of amount of learnable parameters, memory usage, inference time and retrieval accuracy. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.}
%     \label{tab1}
%     %\vskip -0.15in
% % \vspace{-0.2cm}
% \end{table*}

\begin{table*}[!t]
 %\vspace{-0.1cm}
    \centering
    %\footnotesize
    % \vskip 0.1in
    % \renewcommand{\arraystretch}{0.98}
    % \small
    \caption{Comparison results with PETL \textbf{(Top)} and METL \textbf{(Middle, Bottom)} methods on GLUE. Ours${}^\heartsuit$ and Ours${}^\spadesuit$ indicate our method implemented based on UniPT and SHERL, respectively. Best results are in \textbf{bold}, and second best results are \underline{underlined}.}
    \vspace{-0.3cm}
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccccc}
         \toprule[1.2pt]
         \multirow{2}{*}{\centering Method} & Params. & \multicolumn{2}{c}{Memory (G) $\downarrow$} & Time & \multirow{2}{*}{CoLA} & \multirow{2}{*}{SST-2} & \multirow{2}{*}{MRPC} & \multirow{2}{*}{QQP} & \multirow{2}{*}{MNLI} & \multirow{2}{*}{QNLI} & \multirow{2}{*}{RTE} & \multirow{2}{*}{STS-B} & \multirow{2}{*}{Mean} \\
         & (\%) $\downarrow$ & Train & Test & (ms) $\downarrow$ & & & & & & & & & \\
         \midrule[0.6pt]
         \textcolor{gray}{Fully-FT} & \textcolor{gray}{100} & \textcolor{gray}{17.6} & \textcolor{gray}{0.86} & \textcolor{gray}{232.5} & \textcolor{gray}{62.8} & \textcolor{gray}{93.9} & \textcolor{gray}{91.9} & \textcolor{gray}{89.9} & \textcolor{gray}{86.2} & \textcolor{gray}{92.5} & \textcolor{gray}{74.1} & \textcolor{gray}{90.3} & \textcolor{gray}{85.2} \\
         \hline
         Adapter \cite{houlsby2019param} & 1.63 & 13.0 & 0.87 & 247.3 & 64.4 & 94.2 & 88.9 & 88.9 & 86.4 & 93.1 & 75.1 & 91.1 & 85.3 \\
         LoRA \cite{hu2022lora} & 1.71 & 12.6 & 0.86 & 238.1 & 63.3 & 94.3 & 90.1 & 89.0 & 86.3 & 93.2 & 75.5 & 90.9 & 85.3 \\
         BitFit \cite{zaken2022bitfit} & 0.13 & 10.7 & 0.86 & 236.9 & 61.8 & 94.3 & 91.0 & 88.7 & 85.6 & 93.1 & 67.6 & 90.8 & 84.1 \\
         Prompt \cite{li2021prefix} & 0.03 & 22.2 & 0.87 & 291.4 & 0 & 90.3 & 74.6 & 88.5 & 82.5 & 92.5 & 59.5 & 90.1 & 72.2 \\
         \midrule[0.6pt]
         LST \cite{sung2022lst} & 1.74 & 5.5 & 0.88 & 462.7 & 58.1 & 94.1 & 90.4 & 88.8 & \underline{85.6} & 93.3 & \underline{71.9} & 90.7 & 84.1 \\
         UniPT \cite{liao2024uni} & 1.36 & \textbf{2.9} & \textbf{0.86} & 423.6 & \underline{62.2} & \underline{94.2} & \underline{90.8} & 88.9 & 85.5 & 93.3 & 69.8 & 89.7 & 84.3 \\
         SHERL \cite{diao2024sherl} & \textbf{0.85} & \textbf{2.9} & \underline{0.87} & 350.4 & 61.1 & 93.7 & 89.4 & 88.8 & 85.3 & 93.3 & \underline{71.9} & \underline{90.9} & 84.3 \\
         \textbf{Ours${}^\heartsuit$} & 1.48 & \underline{3.3} & \textbf{0.86} & \underline{235.2} & \textbf{62.9} & \textbf{94.4} & \textbf{91.2} & \underline{89.0} & 85.2 & \underline{93.4} & 70.5 & 90.2 & \underline{84.6} \\
         \textbf{Ours${}^\spadesuit$} & \underline{1.02} & 3.4 & \underline{0.87} & \textbf{234.8} & 62.0 & 94.1 & 89.8 & \textbf{89.2} & \textbf{85.7} & \textbf{93.5} & \textbf{72.6} & \textbf{91.2} & \textbf{84.8} \\
         \midrule[0.6pt]
         % \hdashline
         LST~(T5-large) \cite{sung2022lst} & 1.23 & 12.2 & 2.88 & 832.9 & 65.3 & 95.7 & 91.6 & 89.7 & \underline{88.6} & 94.1 & 79.9 & \textbf{92.4} & 87.1 \\
         UniPT~(T5-large) \cite{liao2024uni} & 0.92 & 9.1 & \underline{2.82} & 795.1 & 65.7 & 95.8 & 92.0 & 89.7 & 88.2 & 94.2 & 79.6 & 92.0 & 87.2 \\
         SHERL~(T5-large) \cite{diao2024sherl} & \textbf{0.64} & \textbf{7.1} & \textbf{2.80} & 667.4 & 65.6 & 95.8 & \underline{92.9} & 89.6 & \underline{88.6} & 94.2 & \underline{80.8} & 92.1 & 87.5 \\
         \textbf{Ours${}^\heartsuit$(T5-large)} & 1.02 & 10.2 & \underline{2.82} & \underline{418.7} & \textbf{66.3} & \underline{96.3} & 92.8 & \underline{90.0} & 88.4 & \underline{94.5} & 79.9 & \underline{92.3} & \underline{87.6} \\
         \textbf{Ours${}^\spadesuit$(T5-large)} & \underline{0.81} & \underline{8.0} & \textbf{2.80} & \textbf{415.3} & \underline{66.2} & \textbf{96.5} & \textbf{93.5} & \textbf{90.2} & \textbf{88.9} & \textbf{94.7} & \textbf{81.5} & \textbf{92.4} & \textbf{88.0} \\
         \bottomrule[1.2pt]
    \end{tabular}
    }
    \end{center}
\vspace{-0.2cm}
%    \caption{Comparison results with PETL \textbf{(Top)} and METL \textbf{(Bottom)} methods on GLUE benchmark, with \textit{T5-base/large}. We report the number of learnable parameters and memory usage as efficiency metrics, and accuracy, F1 score, Matthew’s Correlation, and Pearson-Spearman Correlation as performance indicators. Ours${}^\heartsuit$ and Ours${}^\spadesuit$ indicate our method implemented based on the UniPT \cite{diao2024unipt} and SHERL \cite{diao2024sherl}, respectively. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.}    \label{tab_glue_results}
    \label{tab_glue_results}
\end{table*}

\begin{table*}[!ht]
	\centering
     \caption{Comparison results with PETL \textbf{(Top)} and METL \textbf{(Bottom)} methods on VTAB-1K. Best results are in \textbf{bold}, and second best results are \underline{underlined}.}
     \vspace{-0.1cm}
        \small
	\setlength{\tabcolsep}{0.23pt}
	\begin{tabular}{
            p{1.8cm}<{}
            p{0.66cm}<{\centering} p{0.66cm}<{\centering} p{0.9cm}<{\centering}|
            p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}|
            p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}|
            p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}p{0.66cm}<{\centering}| 
            p{0.66cm}<{\centering}
        }
	\toprule[1.5pt]
 
	\multicolumn{4}{c|}{}&\multicolumn{7}{c|}{\textbf{Natural}}&\multicolumn{4}{c|}{\textbf{Specialized}}&\multicolumn{8}{c|}{\textbf{Structured}}&\\
    
        {{\rotatebox{90}{\textbf{Method}}}}
        &{{\rotatebox {90}{Params.~(M) $\downarrow$}}}
        & {{\rotatebox {90}{Memory~(G) $\downarrow$}}}
        &{{\rotatebox {90}{FPS $\uparrow$}}}
	& {{\rotatebox {90}{Cifar100}}}
	& {{\rotatebox {90}{Caltech101}}}
	& {{\rotatebox {90}{DTD}}}
	& {{\rotatebox {90}{Flower102}}}
	& {{\rotatebox {90}{Pets}}}
	& {{\rotatebox {90}{SVHN}}}
	&{{\rotatebox {90}{Sun397}}}
	& {{\rotatebox {90}{Camelyon}}}
	& {{\rotatebox {90}{EuroSAT}}}
	& {{\rotatebox {90}{Resisc45}}}
	&{{\rotatebox {90}{Retinopathy}}}
	& {{\rotatebox {90}{Clevr-Count}}}
	& {{\rotatebox {90}{Clevr-Dist}}}
	& {{\rotatebox {90}{DMLab}}}
	& {{\rotatebox {90}{KITTI-Dist}}}
	& {{\rotatebox {90}{dSpr-Loc}}}
	& {{\rotatebox {90}{dSpr-Ori}}}
	& {{\rotatebox {90}{sNORB-Azim}}}
	&{{\rotatebox {90}{sNORB-Ele}}}
	& {{\rotatebox {90}{\textbf{Mean}}}}\\
 
	\specialrule{0em}{1pt}{1pt}
	\hline
	\specialrule{0em}{1pt}{1pt}
	
	
 
	\textcolor{gray}{Fully-FT} & \textcolor{gray}{85.8} & \textcolor{gray}{6.1} & \textcolor{gray}{89.21} & \textcolor{gray}{68.9} & \textcolor{gray}{87.7} & \textcolor{gray}{64.3} & \textcolor{gray}{97.2} & \textcolor{gray}{86.9} & \textcolor{gray}{87.4} & \textcolor{gray}{38.8} & \textcolor{gray}{79.7} & \textcolor{gray}{95.7} & \textcolor{gray}{84.2} & \textcolor{gray}{73.9} & \textcolor{gray}{56.3} & \textcolor{gray}{58.6} & \textcolor{gray}{41.7} & \textcolor{gray}{65.5} & \textcolor{gray}{57.5} & \textcolor{gray}{46.7} & \textcolor{gray}{25.7} & \textcolor{gray}{29.1} & \textcolor{gray}{68.9} \\
 
	\hline
	
	\specialrule{0em}{1pt}{1pt}
    
    BitFiT & \underline{0.10} & 3.8 & \underline{87.95} & 72.8 & 87.0 & 59.2 & 97.5 & 85.3 & 59.9 & 51.4 & 78.7 & 91.6 & 72.9 & 69.8 & 61.5 & 55.6 & 32.4 & 55.9 & 66.6 & 40.0 & 15.7 & 25.1 & 65.2 \\
    
    VPT & 0.53 & 5.6 & 72.10 & 78.8 & 90.8 & 65.8 & 98.0 & 88.3 & 78.1 & 49.6 & 81.8 & 96.1 & 83.4 & 68.4 & 68.5 & 60.0 & 46.5 & 72.8 & 73.6 & 47.9 & 32.9 & 37.8 & 72.0 \\
    
    RS-Bypass. & 0.42 & {2.4} & 47.53 & 64.5 & 88.8 & 73.2 & 99.4 & 90.6 & 63.5 & \underline{57.2} & 85.5 & 95.2 & 82.4 & 75.2 & 70.4 & 61.0 & 40.2 & 66.8 & 79.2 & 52.6 & 26.0 & \underline{49.3} & 72.3 \\
    
    Adapter & 0.16 & 3.9 & 82.78 & 69.2 & 90.1 & 68.0 & 98.8 & 89.9 & 82.8 & 54.3 & 84.0 & 94.9 & 81.9 & 75.5 & 80.9 & 65.3 & 48.6 & 78.3 & 74.8 & 48.5 & 29.9 & 41.6 & 73.9 \\
    
    LoRA & 0.29 & 3.9 & 85.03 & 67.1 & 91.4 & 69.4 & 98.8 & 90.4 & 85.3 & 54.0 & 84.9 & 95.3 & 84.4 & 73.6 & 82.9 & \textbf{69.2} & 49.8 & 78.5 & 75.7 & 47.1 & 31.0 & 44.0 & 74.5 \\
    
    AdaptFormer & 0.16 & 4.1 & 80.84 & 70.8 & 91.2 & 70.5 & 99.1 & 90.9 & 86.6 & 54.8 & 83.0 & 95.8 & 84.4 & \underline{76.3} & 81.9 & 64.3 & 49.3 & 80.3 & 76.3 & 45.7 & 31.7 & 41.1 & 74.7 \\
    
    NOAH & 0.36 & 5.2 & 56.78 & 69.6 & 92.7 & 70.2 & 99.1 & 90.4 & 86.1 & 53.7 & 84.4 & 95.4 & 83.9 & 75.8 & 82.8 & \underline{68.9} & 49.9 & \underline{81.7} & 81.8 & 48.3 & 32.8 & 44.2 & 75.5 \\
    
    FacT & 0.06 & 4.8 & -- & 70.6 & 90.6 & 70.8 & 99.1 & 90.7 & 88.6 & 54.1 & 84.8 & 96.2 & 84.5 & 75.7 & 82.6 & 68.2 & 49.8 & 80.7 & 80.8 & 47.4 & 33.2 & 43.0 & 75.6 \\
    
    Res-Tuning  & 0.55 & 4.9 & 57.70 & 75.2 & 92.7 & 71.9 & 99.3 & \textbf{91.9} & 86.7 & \textbf{58.5} & 86.7 & 95.6 & 85.0 & 74.6 & 80.2 & 63.6 & 50.6 & 80.2 & 85.4 & 55.7 & 31.9 & 42.0 & 76.3 \\
    
    Convpass & 0.33 & 2.6 & 67.02 & 72.3 & 91.2 & 72.2 & 99.2 & 90.9 & \underline{91.3} & 54.9 & 84.2 & 96.1 & 85.3 & 75.6 & 82.3 & 67.9 & 51.3 & 80.0 & 85.9 & 53.1 & 36.4 & 44.4 & 76.6 \\
    
    \hline
    HST  & 0.78 & 2.8 & 44.17 & 76.7 & \textbf{94.1} & 74.8 & \underline{99.6} & 91.1 & 91.2 & 52.3 & \textbf{87.1} & 96.3 & \textbf{88.6} & \textbf{76.5} & \textbf{85.4} & 63.7 & \textbf{52.9} & \underline{81.7} & \underline{87.2} & 56.8 & 35.8 & \textbf{52.1} & \underline{78.1} \\
    
    LoSA & \textbf{0.05} & \underline{2.1} & {68.92} & \textbf{82.7} & 93.0 & \textbf{76.2} & \textbf{99.7} & 89.8 & 80.0 & 56.1 & 86.3 & \underline{96.7} & 86.7 & \underline{76.3} & 78.8 & 61.4 & 48.0 & \textbf{82.6} & \textbf{91.7} & \textbf{58.4} & \textbf{46.9} & 47.6 & 77.8 \\

    UniPT & 5.19 & \underline{2.1} & 45.72 & 77.4 & 92.9 & 74.8 & \underline{99.6} & 91.6 & 89.7 & 54.9 & \underline{87.0} & 96.5 & 86.9 & 73.8 & 83.8 & 63.7 & 50.9 & 81.4 & 86.5 & 56.4 & 35.9 & 46.8 & 77.4\\

    SHERL & 5.08 & \textbf{2.0} & 48.70 & 78.8 & 93.2 & 75.4 & 99.5 & 91.6 & 90.4 & 55.6 & 86.8 & \underline{96.7} & 87.2 & 75.3 & 84.2 & 63.5 & 51.8 & \underline{81.7} & 86.9 & \underline{57.5} & 36.9 & 48.2 & 77.9 \\
    
    \textbf{Ours} & 5.50 & \underline{2.1} & \textbf{88.89} & \underline{79.8} & \underline{93.6} & \underline{75.7} & 99.5 & \underline{91.8} & \textbf{91.5} & 56.1 & 86.9 & \textbf{96.8} & \underline{87.5} & 75.9 & \underline{84.6} & 64.6 & \underline{52.4} & 81.3 & \underline{87.2} & {57.1} & \underline{37.7} & 47.9 & \textbf{78.3}\\
    

    
	\bottomrule[1.5pt]
	\end{tabular}
%	\caption{Performance Comparison of PETL \textbf{(Top)} and METL \textbf{(Bottom)} methods on VTAB-1K Benchmark across three categories: Natural, Specialized, and Structured datasets. Key metrics include the number of learnable parameters (excluding classification layers), train memory usage, inference time, and accuracy across multiple benchmarks. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.} [origin=c]
	\label{tab_vtab_results}
 % \vspace{-0.2cm}
\end{table*}


% \begin{table*}[!ht]
% 	\centering
% 	\setlength{\tabcolsep}{0.215pt}
% 	\small
% 	\begin{tabular}{
%             p{1.53cm}<{} p{1.75cm}<{\centering}|
%             p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}|
%             p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}|
%             p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}p{0.64cm}<{\centering}| 
%             p{0.64cm}<{\centering} p{0.64cm}<{\centering} p{0.64cm}<{\centering}
%         }
% 	\toprule[1.5pt]
 
% 	\multicolumn{2}{c|}{}&\multicolumn{7}{c|}{\textbf{Natural}}&\multicolumn{4}{c|}{\textbf{Specialized}}&\multicolumn{8}{c|}{\textbf{Structured}}&\\
%         \multicolumn{1}{c}{{\textbf{Method}}}&\multicolumn{1}{c|}{{\textbf{Publication}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Cifar100}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Caltech101}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{DTD}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Flower102}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Pets}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{SVHN}}}
% 	&\multicolumn{1}{c|}{{\rotatebox {90}{Sun397}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Camelyon}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{EuroSAT}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Resisc45}}}
% 	&\multicolumn{1}{c|}{{\rotatebox {90}{Retinopathy}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Clevr-Count}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{Clevr-Dist}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{DMLab}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{KITTI-Dist}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{dSpr-Loc}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{dSpr-Ori}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{sNORB-Azim}}}
% 	&\multicolumn{1}{c|}{{\rotatebox {90}{sNORB-Ele}}}
%         &\multicolumn{1}{c}{{\rotatebox {90}{\textbf{\#Param. (M)}}}}
%         &\multicolumn{1}{c}{{\rotatebox {90}{\textbf{Overall Mean}}}}
% 	&\multicolumn{1}{c}{{\rotatebox {90}{\textbf{Group Mean}}}}\\
 
% 	\specialrule{0em}{1pt}{1pt}
% 	\hline
% 	\specialrule{0em}{1pt}{1pt}
% 	\multicolumn{20}{l}{\emph{Traditional Fine-Tuning Methods}}\\
% 	\hline
% 	\specialrule{0em}{1pt}{1pt}
 
% 	Full& Baseline &68.9&87.7&64.3&97.2&86.9&87.4&38.8&79.7&95.7&84.2&73.9&56.3&58.6&41.7&65.5&57.5&46.7&25.7&29.1 & 85.8 & 65.6 & 68.9 \\
% 	Linear& Baseline &64.4&85.0&63.2&97.0&86.3&36.6&51.0&78.5&87.5&68.5&74.0&34.3&30.6&33.2&55.4&12.5&20.0&9.6&19.2 & 0 & 53.0 & 57.6\\
 
% 	\hline
% 	\specialrule{0em}{1pt}{1pt}
% 	\multicolumn{20}{l}{\emph{PEFT Methods}}\\
% 	\hline
% 	\specialrule{0em}{1pt}{1pt}
%     Adapter & ICML'19 & 69.2 & 90.1 & 68.0 & 98.8 & 89.9 & 82.8 & 54.3 & 84.0 & 94.9 & 81.9 & 75.5 & 80.9 & 65.3 & 48.6 & 78.3 & 74.8 & 48.5 & 29.9 & 41.6 & 0.16 & 71.5 & 73.9\\
    
%     LoRA & ICLR' 22 & 72.9 & 93.4 & 74.7 & 99.4 & 92.0 & 90.7 & 51.7 & 86.5 & 96.7 & 86.7 & 74.3 & 84.8 & 61.7 & 51.8 & 79.7 & 79.9 & 53.0 & 32.6 & 45.7 & 0.17 & 74.1 & 76.4 \\
	
	
% 	\hline
% 	\specialrule{0em}{1pt}{1pt}
	
%     \textbf{FURA} & \textbf{Ours} & 79.2 & 93.7 & \textbf{77.8} & 99.5 & \textbf{92.6} & \textbf{92.0} & 56.6 & 88.2 & 96.4 & \textbf{88.5} & \textbf{76.7} & \textbf{85.1} & 66.8 & \textbf{56.1} & \textbf{83.8} & 88.8 & 55.5 & 33.0 & \textbf{48.7} & 0.17 & \textbf{76.8} & \textbf{78.9} \\
    
% 	\bottomrule[1.5pt]
% 	\end{tabular}
% 	\caption{Comparison}
% 	\label{tab_vtab}
% \end{table*}



\begin{table*}[!t]
% \vspace{-0.2cm}
%     \vskip 0.1in 
    \caption{Comparison results with METL approaches across various architectures and distinct VL tasks. Ours${}^\heartsuit$ and Ours${}^\spadesuit$ denote our implementations based on UniPT and SHERL, respectively. Best results are in \textbf{bold}, and second best results are \underline{underlined}.
    }
    \vspace{-0.2cm}
    \begin{center}
    \setlength{\tabcolsep}{0.36pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c c ccc ccc ccc | c c c ccc ccc}
    \toprule[1.2pt]
    
    \multirow{2}{*}{Method} & Params. & \multicolumn{1}{c}{Mem.} & QPS & \multicolumn{3}{c}{Flickr30K} & \multicolumn{3}{c}{MSCOCO1K} & \multicolumn{3}{c|}{MSCOCO5K} & Params & \multicolumn{1}{c}{Mem.} & QPS & \multicolumn{3}{c}{MSR-VTT} & \multicolumn{3}{c}{MSVD} \\
    
    \cmidrule[0.4pt]{5-13}
    \cmidrule[0.4pt]{17-22}
    & (M) $\!\downarrow$ & (G) $\!\downarrow$ & $\!\uparrow$ & I-T $\!\uparrow\ $ & T-I $\!\uparrow\ $ & Rsum $\!\uparrow\ $ & I-T $\!\uparrow\ $ & T-I $\!\uparrow\ $ & Rsum $\!\uparrow\ $ & I-T $\!\uparrow\ $ & T-I $\!\uparrow\ $ & Rsum $\!\uparrow\ $ & (M) $\!\downarrow$ &  (G) $\!\downarrow$ & $\!\uparrow$ & T-V $\!\uparrow\ $ & V-T $\!\uparrow\ $ & Rsum $\!\uparrow\ $ & T-V $\!\uparrow\ $ & V-T $\!\uparrow\ $ & Rsum $\!\uparrow\ $ \\
    
    \midrule[0.6pt]
    \textcolor{gray}{Fully-FT} & \textcolor{gray}{201.2} & \textcolor{gray}{176.8} & \textcolor{gray}{-} & \textcolor{gray}{85.6} & \textcolor{gray}{73.3} & \textcolor{gray}{546.6} & \textcolor{gray}{83.1} & \textcolor{gray}{71.7} & \textcolor{gray}{542.7} & \textcolor{gray}{64.2} & \textcolor{gray}{51.2} & \textcolor{gray}{468.9} & \textcolor{gray}{151.3} & \textcolor{gray}{48.8} & \textcolor{gray}{-} & \textcolor{gray}{42.8} & \textcolor{gray}{42.1} & \textcolor{gray}{389.2} & \textcolor{gray}{45.2} & \textcolor{gray}{57.1} & \textcolor{gray}{425.5}  \\
    
    \midrule[0.6pt]
    LST \cite{sung2022lst} & \textbf{9.7} & \textbf{24.4} & - & 82.1 & 66.5 & 529.5 & 78.2 & 64.8 & 525.8 & 57.8 & 43.1 & 434.5 & 11.2 & 32.0 & - & 37.0 & 37.8 & 356.7 & 35.5 & 55.4 & 407.2\\
    UniPT \cite{liao2024uni} & 12.4 & \textbf{24.4} & 8.61 & 84.8 & 69.1 & 537.4 & 80.6 & 67.5 & 532.9 & 61.1 & 45.9 & 445.3 & \textbf{9.6} & \textbf{13.6} & 27.03 & 38.9 & 39.3 & 361.3 & 40.9 & 59.7 & 432.1\\
    
    SHERL \cite{diao2024sherl} & \underline{11.3} & \textbf{24.4} & 10.24 & \underline{86.1} & \underline{71.1} & \underline{542.3} & \underline{81.8} & \textbf{69.2} & \underline{537.5} & \underline{62.5} & \underline{47.3} & \underline{450.8} & \textbf{9.6} & \textbf{13.6} & 32.53 & 39.2 & 40.6 & 363.7 & 40.9 & \underline{60.2} & 429.7\\
    
    \textbf{Ours${}^\heartsuit$} & 12.4 & \underline{25.1} & \underline{14.71} & 85.9 & 70.7 & 541.2 & 81.3 & \underline{68.8} & 536.4 & 61.9 & 46.8 & 448.1 & \underline{9.7} & \underline{14.0} & \textbf{43.65} & \underline{40.2} & \underline{40.7} & \underline{365.8} & \underline{42.3} & 60.0 & \underline{435.7}\\
    
    \textbf{Ours${}^\spadesuit$} & 11.4 & {25.2} & \textbf{14.83} & \textbf{86.4} & \textbf{71.6} & \textbf{543.0} & \textbf{82.2} & \textbf{69.2} & \textbf{537.9} & \textbf{63.2} & \textbf{48.0} & \textbf{452.3}& \underline{9.7} & 14.2 & \underline{43.52} & \textbf{40.6} & \textbf{41.2} & \textbf{367.2} & \textbf{42.5} & \textbf{61.3} & \textbf{435.8}\\
    \bottomrule[1.2pt]
    \end{tabular}
    }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c c cc cc | c c c c ccc ccc cc}
    \multirow{2}{*}{Method} & Params. & \multicolumn{1}{c}{Mem.} & Time & \multicolumn{2}{c}{VQAv2} & \multicolumn{2}{c|}{GQA} 
    & Params. & \multicolumn{1}{c}{Mem.} & Time & \multicolumn{3}{c}{RefCOCO} & \multicolumn{3}{c}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg}\\
    
    \cmidrule[0.4pt]{5-8}
    \cmidrule[0.4pt]{12-19}
    & (M) $\!\downarrow$ & (G) $\!\downarrow$ & (ms) $\!\downarrow\ $ & Test$_\text{D}$ $\!\uparrow$ & Test$_\text{S}$ $\!\uparrow$ & Test$_\text{D}$ $\!\uparrow$ & Test$_\text{S}$ $\!\uparrow\ $ & (M) $\!\downarrow$ & (G) $\!\downarrow$ & (ms) $\!\downarrow\ $ & Val $\!\uparrow$ & TestA $\!\uparrow$ & TestB $\!\uparrow$ & Val $\!\uparrow$ & TestA $\!\uparrow$ & TestB $\!\uparrow$ & Val $\!\uparrow$ & Test $\!\uparrow$\\
    
    \midrule[0.6pt]
    \textcolor{gray}{Fully-FT} & \textcolor{gray}{236.8} & \textcolor{gray}{82.0} & \textcolor{gray}{-} & \textcolor{gray}{76.71} & \textcolor{gray}{76.86} & \textcolor{gray}{60.25} & \textcolor{gray}{61.44}& \textcolor{gray}{185.2} & \textcolor{gray}{39.6} & \textcolor{gray}{-} & \textcolor{gray}{86.51} & \textcolor{gray}{89.13} & \textcolor{gray}{81.22} & \textcolor{gray}{79.54} & \textcolor{gray}{84.54} & \textcolor{gray}{70.63} & \textcolor{gray}{80.92} & \textcolor{gray}{80.95} \\
    \midrule[0.6pt]
    LST \cite{sung2022lst} & 13.4 & 25.6 & - & 75.29 & 75.44 & 59.93 & 60.75 & 0.9 & 12.6 & - & 81.63 & 85.19 & 76.03 & 71.32 & 78.20 & 62.06 & 72.53 & 73.67\\
    UniPT \cite{liao2024uni} & \textbf{10.3} & \textbf{11.6} & 106.38 & 75.33 & 75.53 & 60.10 & 60.72 & \textbf{0.7} & \textbf{6.8} & 97.82 & 82.71 & 86.25 & 78.16 & 72.94 & 79.18 & 64.49 & 77.04 & 77.33\\
    SHERL \cite{diao2024sherl} & 13.0 & 14.0 & 92.49 & 75.53 & 75.82 & 60.16 & 60.82 & \textbf{0.7} & \textbf{6.8} & 79.33 & 83.02 & 86.39 & 78.41 & 73.29 & 80.11 & 64.59 & \underline{77.80} & 77.33\\
    
    \textbf{Ours${}^\heartsuit$} & \underline{10.4} & \underline{12.2} & \underline{60.26} & \underline{75.57} & \underline{75.91} & \underline{60.21} & \underline{60.85} & \textbf{0.7} & \underline{7.1} & \underline{52.63} & \textbf{83.11} & \underline{86.64} & \underline{78.69} & \underline{73.49} & \underline{80.15} & \underline{64.72} & 77.49 & \underline{77.73}\\
    
    \textbf{Ours${}^\spadesuit$} & 13.1 & 15.2 & \textbf{59.89} & \textbf{75.88} & \textbf{76.07} & \textbf{60.41} & \textbf{60.93} & \underline{0.8} & \underline{7.1} & \textbf{52.29} & \underline{83.09} & \textbf{86.77} & \textbf{78.97} & \textbf{74.05} & \textbf{80.46} & \textbf{64.79} &\textbf{78.06} & \textbf{78.13}\\
    \bottomrule[1.2pt]
    \end{tabular}
    }
    \end{center}
%     \vskip -0.15in
\vspace{-0.3cm}
        \label{METL-table}
\end{table*}

\begin{table*}[!t]
 %\vspace{-0.1cm}
     \caption{Ablation study on various distillation strategies that are applied to distinct structures (\emph{i.e.} `logits-based' and `feature-based') with different distillation directions, where `S' and `B' refer to side network and backbone, respectively. Best results are in \textbf{bold}, and the second best ones are \underline{underlined}.
    %The best results are highlighted in \textbf{bold}, while the second-best results are \underline{underlined}.
    }
    \centering
    %\footnotesize
    % \vskip 0.1in
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccccccc}
         \toprule[1.2pt]
         \multirow{2}{*}{Method} & {Params.} & {Memory} & {QPS} & \multicolumn{3}{c}{Flickr30K} & \multicolumn{3}{c}{MSCOCO1K} \\
         \cmidrule[0.4pt]{5-10}
         & (M) $\downarrow$ & (G) $\downarrow$ & $\uparrow$ & {I-T} $\uparrow$ & {T-I} $\uparrow$ & {Rsum} $\uparrow$ & {I-T} $\uparrow$ & {T-I} $\uparrow$ & {Rsum} $\uparrow$\\
         \midrule[0.6pt]
         Baseline (UniPT) \cite{liao2024uni} & \textbf{12.4} & \textbf{24.4} & \underline{8.61} & \underline{84.8} & 69.1 & 537.4 & \textbf{80.6} & \underline{67.5} & \textbf{532.9} \\
         \midrule[0.6pt]
         {Logits-based (S$\to$B)} & \textbf{12.4} & \underline{24.7} & \textbf{14.71} & 81.2 & 66.1 & 529.7 & 77.2 & 65.0 & 526.2 \\
         \midrule[0.3pt]
         {Feature-based (B$\to$S)} & \textbf{12.4} & \underline{24.7} & \textbf{14.71} & 81.9 & 66.5 & 531.5 & 78.3 & 65.9 & 528.1 \\
         \midrule[0.3pt]
         {Feature-based (S$\to$B)} & \textbf{12.4} & \underline{24.7} & \textbf{14.71} & 78.9 & 63.0 & 518.2 & 73.1 & 60.9 & 508.3 \\
         \midrule[0.3pt]
         \textbf{Ours} (B $\leftrightarrows$ S) & \textbf{12.4} & 25.1& \textbf{14.71} & \textbf{84.9} & \textbf{69.5} & \textbf{538.1} & 80.2 & \textbf{67.7} & \underline{532.7} \\
         \bottomrule[1.2pt]
    \end{tabular}
% \vspace{-0.2cm}
    \label{tab_ablation_distillation}
\end{table*}

\begin{table*}[!t]
 %\vspace{-0.1cm}
     \caption{Ablation study on fading the side network during inference on distinct datasets for the ITR task. Best results are in \textbf{bold}, and the second best ones are \underline{underlined}.}
    \centering
    %\footnotesize
    % \vskip 0.1in
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccccc}
         \toprule[1.2pt]
         \multirow{2}{*}{Method} & Fading & {Params.} & {Memory} & {QPS} & \multicolumn{3}{c}{Flickr30K} & \multicolumn{3}{c}{MSCOCO1K} \\
         \cmidrule[0.4pt]{6-11}
         & Side Network & (M) $\downarrow$ & (G) $\downarrow$ & $\uparrow$ & {I-T} $\uparrow$ & {T-I} $\uparrow$ & {Rsum} $\uparrow$ & {I-T} $\uparrow$ & {T-I} $\uparrow$ & {Rsum} $\uparrow$\\
         \midrule[0.6pt]
         \textcolor{gray}{Fully-FT} & \textcolor{gray}{$\times$} & \textcolor{gray}{201.2} & \textcolor{gray}{176.8} & \textcolor{gray}{-} & \textcolor{gray}{85.6} & \textcolor{gray}{73.3} & \textcolor{gray}{546.6} & \textcolor{gray}{83.1} & \textcolor{gray}{71.7} & \textcolor{gray}{542.7} \\
         LST \cite{sung2022lst} & $\times$ & \textbf{9.7} & \textbf{24.4} & - & 82.1 & 66.5 & 529.5 & 78.2 & 64.8 & 525.8 \\ 
         \midrule[0.6pt]
         UniPT \cite{liao2024uni} & $\times$ & 12.4 & \textbf{24.4} & 8.61 & 84.8 & 69.1 & 537.4 & 80.6 & 67.5 & 532.9\\

         \multirow{2}{*}{\textbf{\textbf{Ours${}^\heartsuit$}}} & $\times$ & 12.4 & \underline{25.1} & 7.98 & 86.2 & 70.9 & 541.9 & 81.8 & \underline{69.4} & 537.6\\

         & \checkmark & 12.4 & \underline{25.1} & \underline{14.71} & 85.9 & 70.7 & 541.2 & 81.3 & {68.8} & 536.4\\
         \midrule[0.6pt]
         SHERL \cite{diao2024sherl} & $\times$ & \underline{11.3} & \textbf{24.4} & 10.24 & {86.1} & {71.1} & \underline{542.3} & \underline{81.8} & {69.2} & {537.5}\\

         \multirow{2}{*}{\textbf{Ours${}^\spadesuit$}} & $\times$ & 11.4 & 25.2 & 9.76 & \textbf{87.0} & \underline{71.4} & \textbf{543.9} & \textbf{82.5} & \textbf{69.8} & \textbf{539.0}\\
         
         & \checkmark & 11.4 & {25.2} & \textbf{14.83} & \underline{86.4} & \textbf{71.6} & \underline{543.0} & \underline{82.2} & {69.2} & \underline{537.9}\\
         \bottomrule[1.2pt]
    \end{tabular}
% \vspace{-0.2cm}
    \label{tab_ablation_fading}
\end{table*}

\subsection{Main Results}
Following \cite{diao2024unipt}, we compare MDPD against state-of-the-art PETL and METL methods, while Fully Fine-Tuning (Fully-FT) and Partially tuning baselines without comparison. 
\subsubsection{Our Method vs. PETL Approaches}
%As adopted in \cite{diao2024unipt}, the compared memory inefficient PETL approaches include: 1) Selective Tuning methods that optimizes an extremtely small subset of parameters in pre-trained models (\emph{e.g.} bias terms, scaling factors, normalization layers) while keeping the rest ones frozen, such as Adapter \cite{houlsby2019param}, BitFit \cite{zaken2022bitfit}, SSF \cite{lian2022scaling}, and FacT \cite{jie2023fact}; 2) Addictive Tuning methods that introduces learnable prompt vectors into the input sequence, such as Prompt \cite{li2021prefix}; 3) Reparameterized Tuning methods that employs additional low-rank trainable parameters for fine-tuning, such as LoRA \cite{hu2022lora}, AdaLoRA \cite{zhang2023adaptive}; In VTAB-1K benchmark, we expand our methodology by incorporating additional approaches,including the latest state-of-the-art (SOTA) methods, such as HST \cite{lin2023hierarchical} and LoSA \cite{mercea2024time}.
% Similar to \cite{diao2024unipt}, 
{We compare to the following approaches without adopting memory reduction strategies}: 1) Selective Tuning methods including BitFit \cite{zaken2022bitfit}, and FacT \cite{jie2023fact}; 2) Additive Tuning methods including Prompt \cite{li2021prefix}, Adapter \cite{houlsby2019param}, AdaptFormer \cite{chen2022adaptformer}, NOAH \cite{zhang2024neural}, Convpass \cite{jie2024convolutional}, Res-Tuning \cite{jiang2024res}; 3) Re-parameterized Tuning methods including LoRA \cite{hu2022lora}, SSF \cite{lian2022scaling}, AdaLoRA \cite{zhang2023adaptive}. On VTAB-1K benchmark, we additionally compare with VPT \cite{jia2022visual}.
%HST \cite{lin2023hierarchical} and LoSA \cite{mercea2024time}.

\textbf{Results on VL Tasks.} 
% Following \cite{diao2024unipt}, 
We employ two structures from \textit{VSE$\infty$} \cite{chen2021VSE} with BERT-base+BUTD regions and ResNeXt-101+BiGRU for ITR, and one structure from \textit{CLIP4Clip} \cite{luo2021clip4clip} with ViT-base+Text Transformer for VTR. As shown in Table~\ref{tab1}, our method promotes accuracy of compared PETL approaches in most cases. Despite adopting slightly more learnable parameters, our method substantially reduces training memory overhead, by least 59.5\%, 90.4\% and 64.3\% with various backbones respectively, through optimizing lightweight side networks instead of backbones. It also yields the highest retrieval rate and the fastest inference time by abandoning side networks after training.
% \indent- \textit{VSE$\infty$} with ResNeXt-101 \cite{xie2017aggregated} (32$\times$8d) + a BiGRU \cite{schuster1997bidirectional} (tiny);\\
% \indent- \textit{VSE$\infty$} with BERT-base \cite{devllin2019bert} + BUTD regions \cite{anderson2018bottom} (tiny);\\
% \indent- ViT-base \cite{alexey2021vit} and a Text Transformer \cite{radford2019language}.

%As displayed in Table~\ref{tab1}, our method achieves the highest accuracy in most cases and delivers competitive performance in the remaining scenarios. Meanwhile, despite employing slightly more learnable parameters, our method substantially reduces the memory overhead during training by leveraging the side network for back-propagation instead of the large-scale backbone, while maintaining the lowest inference time cost via abandoning the auxiliary side networks without compromising accuracy. For instance, our method deceases the training memory usage of compared PETL approaches by at least 59.5\%, 90.4\% and 64.3\% for BERT, ResNeXt-101 and ViT+Text Transformer settings, respectively. These results underscore the broad applicability and efficiency of our approach with high accuracy across diverse architectures and tasks. 


\textbf{Results on Language-only Tasks.}
Table~\ref{tab_glue_results} shows the performance on GLUE with T5-base \cite{raffel2020exploring} by default. Our method decreases training memory by at least 68.2\% and reaches the minimal inference latency compared to PEFT approaches, while maintaining competitive accuracy with 
comparable trainable parameters. When incorporating T5-large, our method promotes accuracy of PETL methods by a large margin with lower memory usage. 

%\cite{zaken2022bitfit,jia2022visual,jiang2024res,houlsby2019param,hu2022lora,chen2022adaptformer,zhang2024neural,jie2023fact,jie2024convolutional,lin2023hierarchical,mercea2024time}

\textbf{Results on Vision-only Tasks.}
We evaluate the performance of our method for vision-only tasks on VTAB-1K benchmark by adopting a ViT-B pre-trained on ImageNet-21K. As summarized in Table~\ref{tab_vtab_results}, our method achieves a new SOTA performance on average across 19 datasets. Benefiting from side network with dual path knowledge distillation, our method is clearly more memory efficient than compared PETL approaches, reducing the training memory usage, while maintaining the least inference time cost.
%In terms of computational efficiency, our approach is 22.5\% faster than the second-best METL method, LoSA, demonstrating a strong balance between performance and speed. 

% \begin{table*}[!t]
%  %\vspace{-0.1cm}
%     \centering
%     %\footnotesize
%     % \vskip 0.1in
%     \small
%     \begin{center}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ccccccccccc}
%          \toprule[1.2pt]
%          \multirow{2}{*}{Method} & \multirow{2}{*}{Bottleneck} & {Params.} & {Memory} & {Time} & \multicolumn{3}{c}{Flickr30K} & \multicolumn{3}{c}{MSCOCO1K} \\
%          \cmidrule[0.4pt]{6-11}
%          & & (M) \downarrow & (G) \downarrow & (ms) \downarrow & {I-T} \uparrow & {T-I} \uparrow & {Rsum} \uparrow & {I-T} \uparrow & {T-I} \uparrow & {Rsum} \uparrow\\
%          \midrule[0.6pt]
%          Baseline (UniPT) & - & \textbf{12.4} & \textbf{15.1} & 116.21 & \underline{84.8} & 69.1 & 537.4 & \textbf{80.6} & \underline{67.5} & \textbf{532.9} \\
%          \midrule[0.6pt]
%          \multirow{2}{*}{Logits-based (S$\to$B)} & $\times$ & \underline{15.3} & \underline{15.7} & \textbf{61.01} & 81.8 & 66.5 & 530.3 & 77.8 & 65.6 & 527.1 \\
%          & \checkmark & \textbf{12.4} & \underline{15.7} & \underline{67.98} & 81.2 & 66.1 & 529.7 & 77.2 & 65.0 & 526.2 \\
%          \midrule[0.3pt]
%          \multirow{2}{*}{Feature-based (B$\to$S)} & $\times$ & 20.9 & \underline{15.7} & \textbf{61.01} & 82.4 & 67.1 & 532.4 & 78.9 & 66.4 & 529.6 \\
%          & \checkmark & \textbf{12.4} & \underline{15.7} & \underline{67.98} & 81.9 & 66.5 & 531.5 & 78.3 & 65.9 & 528.1 \\
%          \midrule[0.3pt]
%          \multirow{2}{*}{Feature-based (S$\to$B)} & $\times$ & 20.9 & \underline{15.7} & \textbf{61.01} & 79.4 & 63.7 & 519.5 & 73.9 & 62.1 & 510.6 \\
%          & \checkmark & \textbf{12.4} & \underline{15.7} & \underline{67.98} & 78.9 & 63.0 & 518.2 & 73.1 & 60.9 & 508.3 \\
%          \midrule[0.3pt]
%          Logits-based + Feature-based & $\times$ & 20.9 & 15.9 & \textbf{61.01} & 84.7 & \underline{69.2} & \underline{537.5} & \underline{80.3} & 67.1 & 532.1 \\
%          (B $\leftrightarrows$ S) & \checkmark & \textbf{12.4} & 15.9 & \underline{67.98} & \textbf{84.9} & \textbf{69.5} & \textbf{538.1} & 80.2 & \textbf{67.7} & \underline{532.7} \\
%          \bottomrule[1.2pt]
%     \end{tabular}
%     }
%     \end{center}
% % \vspace{-0.2cm}
%     \caption{Ablation study on various distillation strategies, focusing on different types of knowledge (logits- and feature-based) and the direction of feature distillation, represented by directional arrows. The column 'bottleneck' denotes whether a bottleneck structure is employed to align the teacher and student features during feature distillation. The best results are highlighted in \textbf{bold}, while the second-best results are \underline{underlined}.}    \label{tab_ablation_distillation}
% \end{table*}

% \begin{table}[!t]
%  %\vspace{-0.1cm}
%     \centering
%     % \vskip 0.1in
%     \small
%     \begin{center}
%     % \resizebox{\textwidth}{!}
%     {
%     \begin{tabular}{cccccccccc}
%          \toprule[1.2pt]
%          \multirow{2}{*}{Method} & {Params.} & {Memory} & {Time} & \multicolumn{3}{c}{Flickr30K} & \multicolumn{3}{c}{MSCOCO1K} \\
%          \cmidrule[0.4pt]{6-11}
%          & (M) \downarrow & (G) \downarrow & (ms) \downarrow & {I-T} \uparrow & {T-I} \uparrow & {Rsum} \uparrow & {I-T} \uparrow & {T-I} \uparrow & {Rsum} \uparrow\\
%          \midrule[0.6pt]
%          Baseline (UniPT) & \textbf{12.4} & \textbf{15.1} & 116.21 & \underline{84.8} & 69.1 & 537.4 & \textbf{80.6} & \underline{67.5} & \textbf{532.9} \\
%          \midrule[0.6pt]
%          \multirow{2}{*}{Logits-based (S$\to$B)} & \underline{15.3} & \underline{15.7} & \textbf{61.01} & 81.8 & 66.5 & 530.3 & 77.8 & 65.6 & 527.1 \\
%           & \textbf{12.4} & \underline{15.7} & \underline{67.98} & 81.2 & 66.1 & 529.7 & 77.2 & 65.0 & 526.2 \\
%          \midrule[0.3pt]
%          \multirow{2}{*}{Feature-based (B$\to$S)} & 20.9 & \underline{15.7} & \textbf{61.01} & 82.4 & 67.1 & 532.4 & 78.9 & 66.4 & 529.6 \\
%          & \textbf{12.4} & \underline{15.7} & \underline{67.98} & 81.9 & 66.5 & 531.5 & 78.3 & 65.9 & 528.1 \\
%          \midrule[0.3pt]
%          \multirow{2}{*}{Feature-based (S$\to$B)} & 20.9 & \underline{15.7} & \textbf{61.01} & 79.4 & 63.7 & 519.5 & 73.9 & 62.1 & 510.6 \\
%          & \textbf{12.4} & \underline{15.7} & \underline{67.98} & 78.9 & 63.0 & 518.2 & 73.1 & 60.9 & 508.3 \\
%          \midrule[0.3pt]
%          Logits-based + Feature-based & 20.9 & 15.9 & \textbf{61.01} & 84.7 & \underline{69.2} & \underline{537.5} & \underline{80.3} & 67.1 & 532.1 \\
%          (B $\leftrightarrows$ S) & \textbf{12.4} & 15.9 & \underline{67.98} & \textbf{84.9} & \textbf{69.5} & \textbf{538.1} & 80.2 & \textbf{67.7} & \underline{532.7} \\
%          \bottomrule[1.2pt]
%     \end{tabular}
%     }
%     \end{center}
% % \vspace{-0.2cm}
%     \caption{Ablation study on various distillation strategies, focusing on different types of knowledge (logits- and feature-based) and the direction of feature distillation, represented by directional arrows. The column 'bottleneck' denotes whether a bottleneck structure is employed to align the teacher and student features during feature distillation. The best results are highlighted in \textbf{bold}, while the second-best results are \underline{underlined}.}    \label{tab_ablation_distillation}
% \end{table}

\subsubsection{Our Method vs. METL Approaches}
We further compare with SOTA METL approaches, including LST \cite{sung2022lst}, UniPT \cite{diao2024unipt}, SHERL \cite{diao2024sherl}, HST \cite{lin2023hierarchical} and LoSA \cite{mercea2024time}. It is worth noting that not all compared methods are fully evaluated on the selected benchmarks. Particularly, UniPT and SHERL did not report results on VTAB-1K. We therefore reproduce their results by using the released source code, while adopting the reported results for the others. As shown in Tables~\ref{tab1}-\ref{tab_vtab_results}, our method consistently promotes accuracy of existing METL methods through mutually distilling backbones and side networks across multiple layers with fine-grained distillation strategies. For instance, in Table~\ref{tab1}, we suppresses LST/UniPT by average gains of 3.4\%/1.4\% in R@1 and 11.9\%/5.7\% in Rsum on cross-model retrieval.

%also compare our method with best METL counterparts on language-only tasks in Table~\ref{tab_glue_results}}, and observe that it consistently exceeds other METL works across diverse scales of T5-series with comparable trainable parameter and memory usage, while gains a better performance with saving 39.3\% and 43.1\% inference time overhead on T5-base and T5-large, respectively.
Additionally, we expand evaluations for VL tasks on more downstream datasets and network architectures including VSE$\infty$~\cite{chen2021VSE}, CLIP4Clip~\cite{luo2021clip4clip}, CLIP-ViL~\cite{shen2021much} and MDETR~\cite{kamath2021mdetr}, of which details are depicted in \emph{Supplementary Material}. As shown in Table~\ref{METL-table}, MDPD clearly promotes accuracy of compared METL method across various VL tasks by maintaining almost same training memory overhead. Particularly, based on UniPT/SHERL, our method achieves an average improvement of 1.0/0.7\% in R@1 and 3.6/2.4\% in Rsum for cross-modal retrieval, about 0.86/0.96\% improvements on QA task, and total benefits of 3.92/3.38\% for VG task, respectively. Moreover, benefiting from the design of our side branch that is utilized only for training and is abandoned during inference, our method remarkably accelerates the inference speed. Notably, our method decreases the inference time cost of SHERL by at least 25.2\%, clearly showing the efficiency of our method.

%\indent -\textit{VSE$\infty$} \cite{chen2021VSE} with BERT-base \cite{devllin2019bert} model and ResNeXt-101(32$\times$8d) \cite{xie2017aggregated} backbone pre-trained on Instagram (WSL) on Flickr30K, MSCOCO1K and MSCOCO5K for the \textbf{ITR} task;

%\indent -\textit{CLIP4Clip} \cite{luo2021clip4clip} with the pre-trained CLIP \cite{radford2021learning} using Text Transformer \cite{radford2019language} and ViT-B/32 \cite{alexey2021vit} on MSR-VTT and MSVD for the \textbf{VTR} task;

%\indent -\textit{CLIP-ViL} \cite{shen2021much} that applies the CLIP image backbone \cite{radford2021learning} and encodes the text into word embeddings, followed by a cross-modal Transformer on VQAv2 and GQA for the \textbf{QA} task;

%\indent -\textit{MDETR} \cite{kamath2021mdetr} that integrates a pre-trained ResNet-101, RoBERTa-base \cite{liu2019roberta} with an encoder-decoder Transformer on RefCOCO, RefCOCO+ and RefCOCOg for the \textbf{VG} task.




%As summarized in Table~\ref{METL-table}, our method consistently delivers superior accuracy compared to the METL approaches across various multi-modal tasks by maintaining almost the same memory usage, greatly reducing the gap between fully fine-tuning and METL methods, even rivaling or surpassing the performance of fully fine-tuning in many cases. Specifically, our method achieves an average improvement of 1.2\% on R@1 and 0.6\% on Rsum for the ITR and VTR tasks, compared with the second best SHERL approach. Moreover, our method obtains average improvements of 0.3\% and 0.5\% for the QA task and VG task, respectively, by leveraging the elaborately designed dual path distillation strategy. Moreover, benefiting from the design of our bypass branch that is utilized only for training and is abandoned during inference, our method significantly accelerate the inference speed. Notably, our method decreases the inference time cost of the state-of-the-art SHERL method by at least 25.2\%. These results demonstrate the effectiveness and efficiency of our approach across diverse multi-modal tasks.

%Our method demonstrates significant advantages over existing approaches, consistently delivering superior performance across various multi-modal tasks while maintaining efficiency comparable to the state-of-the-art SHERL. In many aspects, it rivals or even surpasses the performance of fully fine-tuned models. Specifically, for cross-modal retrieval tasks (i.e., ITR and VTR), our SHERL-based method achieves an average improvement of 1.2\% on R@1 and 0.6\% on Rsum over SHERL, showcasing its enhanced retrieval capabilities. Additionally, on the QA task, it attains an average improvement of 0.3\%, while on the VG task, it demonstrates an average increase of 0.5\%.  A key advantage of our approach lies in the design of the bypass branch, which is not required during inference, significantly boosting inference speed. Our method reduces inference time by an average of 32.1\% compared to SHERL. These results highlight the effectiveness and efficiency of our approach in addressing diverse multi-modal learning challenges



\subsection{Ablation Study}

\textbf{Effect of Dual Path Knowledge Distillation.}
Our method introduces a dual-path distillation framework that integrates both feature-based distillation from backbone to side network and logits-based distillation from side network to backbone. To validate the effectiveness of the approach, we compare different distillation strategies. As shown in Table~\ref{tab_ablation_distillation}, the combination of logits- and feature-based distillation consistently outperforms compared strategies, highlighting their complementary benefits. Additionally, utilizing a bottleneck for feature-based distillation significantly reduces the amount of learnable parameters and training memory without sacrificing the accuracy. The dual path distillation, which combines both logits- and feature-based distillation, proves essential for achieving SOTA performance while maintaining computational efficiency.

\textbf{Effect of Fading the Side Network in Inference.}
To further clarify the influence of fading the side network on performance during inference, we conduct ablation study by comparing with state-of-the-art METL approaches. As shown in Table~\ref{tab_ablation_fading}, when adopting both the backbone and side network, our method achieves improvements of 13.0\%, 4.6\% and 1.6\% in Rsum compared to LST \cite{sung2022lst}, UniPT \cite{liao2024uni} and SHERL \cite{diao2024sherl}, respectively, under comparable efficiency including the number of trainable parameters, memory usage and inference time. Furthermore, by discarding the side network during inference, our method significantly gains at least 44.8\% improvement in queries per second, with a slight performance decrease of about 0.9\%. The results clearly demonstrate the effectiveness of fading the side branch, when applying our proposed approach.

We also extensively study the hierarchical feature-based distillation module, including \textbf{influence of the mask ratio $\bm{\lambda}$} in Eq.~\eqref{eq:mask}, \textbf{effect of generation block $\bm{\mathcal{G}}$} in Eq.~\eqref{eq:generation_block} and \textbf{impact of feature distillation loss} on distinct layers. Due to space limitation, we summarize the detailed results in \emph{Supplementary Material}. 



==> CVPR26_MDPD/main_sec/5_conclusion.tex <==
\section{Conclusion}
In this paper, we propose a novel approach dubbed Masked Dual Path Distillation (MDPD) to accelerate the memory-efficient transfer learning based on side networks. Specifically, MDPD leverages the features of side networks to efficiently guide the fine-tuning of a small number of parameters of backbone during training, and abandons side networks during inference. To maintain the accuracy, we propose a Hierarchical Feature-based Distillation strategy to enhance the optimization of backbones. We extensively evaluate the performance of MDPD on various pre-trained models across the vision-language and vision/language-only tasks. The results reveal that our method remarkably reduce the inference time, while maintaining the accuracy as well as the memory and parameter efficiency.

==> CVPR26_MDPD/main_sec/6_acknowledgment.tex <==
\section*{Acknowledgments}
\label{sec:acknowledgments}
% TODO Acknowledgments here
{This work was partly supported by the Beijing Natural Science Foundation (No. 4242044 and No. L259044), the CCF Baidu Open Fund, and the Fundamental Research Funds for the Central Universities.}

==> CVPR26_MDPD/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\usepackage{amsfonts}
% \usepackage{mathtools}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{amsmath}
% \usepackage{graphicx}
\usepackage{amssymb}
\usepackage{pifont}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage[accsupp]{axessibility}
% \usepackage{arydshln}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}
